GA-NIFS: The highly overdense system BR1202-0725 at z $\sim$ 4.7. A double AGN with fast outflows plus eight companion galaxies

Distant quasars (QSOs) in galaxy overdensities are considered key actors in the evolution of the early Universe. In this work, we studied the kinematic and physical properties of the BR1202-0725 system at z=4.7, one of the most overdense fields known in the early Universe, consisting of a QSO, a submillimeter galaxy (SMG), and three Lyman-$\alpha$ emitters. We used data from the JWST/NIRSpec Integral Field Unit (IFU) to analyze the rest-frame optical emission of each source in the system. We estimated a bolometric luminosity of log($L_{\rm bol}/$[erg/s]) = 47.2 $\pm$ 0.4 and a black hole mass of log($M_{\rm BH}/M_\odot$) = 10.1 $\pm$ 0.5 for the QSO, which are consistent with previous measurements obtained with ground-based observations. The NIRSpec spectra of the SMG revealed instead unexpected [OIII] and H$\alpha$+[NII] profiles. The overall [OIII] line profile is blue-shifted by more than 700 km/s relative to the systemic velocity of the galaxy. Additionally, both the [OIII] and H$\alpha$+[NII] lines show prominent broad (1300 km/s), blueshifted wings associated with outflowing ionized gas. The analysis of NIRSpec and X-ray observations indicates that the SMG likely hosts an accreting supermassive black hole as supported by the following results: (i) the excitation diagnostic diagram is consistent with ionization from an active galactic nucleus (AGN); (ii) the X-ray luminosity is higher than $10^{44}$ erg/s; and (iii) it hosts a fast outflow ($v_{\rm out}$ = 5000 km/s), comparable to those observed in luminous QSOs. Therefore, the QSO-SMG pair represents one of the highest-redshift double AGN to date, with a projected separation of 24 kpc. Finally, we investigated the environment of this system and found four new galaxies at the same redshift of the QSO and within a projected distance of 5 kpc from it. This overdense system includes at least ten galaxies in only 980 kpc$^2$.

==> Masses.tex <==
\subsection{\textbf{Dynamical masses of the system}}
%The newly discovered galaxies have velocities relatively close in projection, in a range of $\sim$ 1000 \kms, and close to the one of the QSO (see Tab. \ref{tab:Comp}). Then, the mass of the halo must be very large and we can calculated the dynamical masses for each observed galaxy companion from its measured velocity dispersion and size. 

\textbf{We estimate the dynamical masses of the sources in the system assuming a virialised system and using the expression given by \cite{ho1996a,ho1996b}:}
\begin{equation}
M^{dyn}=K\cdot \sigma^2 \cdot \frac{R}{G}
\end{equation}
\textbf{where K is a factor that depends on the mass distribution in the galaxy \citep[assumed as K = 5, see][]{cappellari2006}, $\sigma$ is the one-dimensional velocity dispersion of the system, R is its radius and G is the gravitational constant.}

\textbf{The integrated velocity dispersion has been calculated using the narrow component results of each source, which has been corrected for instrumental broadening. Additionally, we have used the results from \citet{bezanson2018} to take into account the differences in the integrated velocity dispersion of the ionised gas and the stars (see its Fig. 4b). The mean velocity dispersion of the LAEs and companions is $\sim$ 170 \kms (see Tab. \ref{tab:Comp}), then the correction is $\Delta$log($\sigma$[\kms]) $\sim$ 0. For the SMG and QSO narrow components %($\sigma$ = 471 \kms and 356 \kms)
this correction is $\Delta$log($\sigma$[\kms]) =  0.2. Then, we have used $\sigma_{SMG}^*$ = 297 $\pm$ 13 \kms and $\sigma_{QSO}^*$ = 224 $\pm$ 15 \kms. }


\textbf{The size of each source is difficult to measure. Then, for the QSO host galaxy we have assumed a typical size of 2 kpc. For the SMG we have fitted an elliptical profile, with a semi major axis of 2.75 kpc. For the two sources in LAE1 we have assumed the semi major axis of each one (2.92 kpc and 3.56 kpc for LAE1a and LAE1b respectively, see Fig. \ref{fig:fmapLae1}), for the LAE2 and the four galaxy companions we have assumed the size of the apertures used in the analysis. It is important to emphasize that these sizes has been measured in ionised gas, which would have an extension larger than the stellar component of each galaxy. Then, we cal consider the dynamical masses calculated as higher limits.}



==> SMG/Fitting_SMG.tex <==
\begin{table*}[h]
    \centering
    \caption{SMG emission line velocity and velocity dispersions in km/s for each component. Emission line intensities (10$^{-20}$ erg/s/cm$^2$).}
    \begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}ccc}
    \hline 
    \multicolumn{3}{c}{Scenario 1}\\
        \hline \hline
        ~ & $\sigma$ (km/s) & v (km/s)$^a$\\ \hline \hline
        Narrow 1 & 471 $\pm$ 20 &  111 $\pm$ 2\\ 
        Narrow 2 & 300 $\pm$ 102 &  -762 $\pm$ 89 \\ 
        Outflow &  1291 $\pm$ 537 &  -2445 $\pm$ 37\\       
\hline
    \end{tabular*}\\
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}ccccc}
\hline
Line & $\lambda$ & Narrow 1 & Narrow 2 & Outflow \\
\hline \hline
$[OIII]$ & 5007 & - & 80 $\pm$ 25 & 16 $\pm$ 12\\

$H\alpha$ & 6563 & 11 $\pm$ 2  & 6 $\pm$ 2 & -\\
$[NII]$ & 6584 &  45 $\pm$ 2 & 8 $\pm$ 3 & 45 $\pm$ 1 \\
$[SII]$ & 6717 & -  &  3 $\pm$ 1  & - \\
$[SII]$ & 6731 & - &  1 $\pm$ 1  & - \\
\hline
\end{tabular*}\\
\vspace*{10px}










\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}ccc}
    \hline 
    \multicolumn{3}{c}{Scenario 2}\\
        \hline \hline
        ~ & $\sigma$ (km/s) & v (km/s)$^a$\\ \hline \hline
        Narrow 1 & 471 $\pm$ 18 &  72 $\pm$ 2\\ 
        Narrow 2 & 300 $\pm$ 102 &  -762 $\pm$ 89 \\ 
        Outflow &  1291 $\pm$ 537 &  -2445 $\pm$ 37\\     
        BLR &  1372	 $\pm$ 48 &  -1614 $\pm$ 430\\       
\hline
    \end{tabular*} 	\\
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}cccccc}
\hline
Line & $\lambda$ & Narrow 1 & Narrow 2 & BLR & Outflow\\
\hline \hline
$[OIII]$ & 5007 & - & 80 $\pm$ 25 & - & 16 $\pm$ 12\\

$H\alpha$ & 6563 &  11 $\pm$ 1   &  4 $\pm$ 1  &  16 $\pm$ 2 & -  \\
$[NII]$ & 6584 &   45 $\pm$ 1 &  5 $\pm$ 2 & - & -  \\
$[SII]$ & 6717 &   -   &   3 $\pm$ 1   & - & -  \\
$[SII]$ & 6731 &  -  &   1 $\pm$ 1   & - & -  \\
\hline
\end{tabular*}

\begin{tablenotes}
\item $^a$ Acording to z = 4.6891 \citep{2013A&A...559A..29C}.\\
\end{tablenotes}





\label{tab:SMG}
\end{table*}

==> SMG/Fitting_vel.tex <==
\begin{table}[h]
    \centering
    \caption{SMG emission line velocity and velocity dispersions in km/s for each component. Emission line intensities (10$^{-20}$ erg/s/cm$^2$).}
    \begin{tabular}{ccc}
    \hline 
    \multicolumn{3}{c}{Scenario 1}\\
        \hline \hline
        ~ & $\sigma$ (km/s) & v (km/s)$^a$\\ \hline \hline
        Narrow 1 & 471 $\pm$ 20 &  111 $\pm$ 2\\ 
        Narrow 2 & 300 $\pm$ 102 &  -762 $\pm$ 89 \\ 
        Outflow &  1291 $\pm$ 537 &  -2445 $\pm$ 37\\       
\hline
    \end{tabular}
\begin{tabular}{ccccc}
\hline
\hline
Line & $\lambda$ & Narrow 1 & Narrow 2 & Outflow \\
\hline \hline
$[OIII]$ & 5007 & - & 80 $\pm$ 25 & 16 $\pm$ 12\\

$H\alpha$ & 6563 & 11 $\pm$ 2  & 6 $\pm$ 2 & -\\
$[NII]$ & 6584 &  45 $\pm$ 2 & 8 $\pm$ 3 & 45 $\pm$ 1 \\
$[SII]$ & 6717 & -  &  3 $\pm$ 1  & - \\
$[SII]$ & 6731 & - &  1 $\pm$ 1  & - \\
\hline
\end{tabular}

\begin{tablenotes}
\item $^a$ Acording to z = 4.6891 \citep{2013A&A...559A..29C}.\\
\end{tablenotes}  

\label{tab:SMG1}
\end{table}

==> SMG/Fitting_vel_BLR.tex <==
\begin{table}[h]
    \centering
    \caption{SMG (scenario 2) emission line velocity and velocity dispersions in km/s for each component. Emission line intensities (10$^{-20}$ erg/s/cm$^2$).}
    \begin{tabular}{ccc}
    \hline 
    \multicolumn{3}{c}{Scenario 2}\\
        \hline \hline
        ~ & $\sigma$ (km/s) & v (km/s)$^a$\\ \hline \hline
        Narrow 1 & 471 $\pm$ 18 &  72 $\pm$ 2\\ 
        Narrow 2 & 300 $\pm$ 102 &  -762 $\pm$ 89 \\ 
        BLR &  1372	 $\pm$ 48 &  -1614 $\pm$ 430\\       
\hline
    \end{tabular} 	
\begin{tabular}{cccccc}
\hline
\hline
Line & $\lambda$ & Narrow 1 & Narrow 2 & BLR & Outflow\\
\hline \hline
$[OIII]$ & 5007 & - & 80 $\pm$ 25 & - & 16 $\pm$ 12\\

$H\alpha$ & 6563 &  11 $\pm$ 1   &  4 $\pm$ 1  &  16 $\pm$ 2 & -  \\
$[NII]$ & 6584 &   45 $\pm$ 1 &  5 $\pm$ 2 & - & -  \\
$[SII]$ & 6717 &   -   &   3 $\pm$ 1   & - & -  \\
$[SII]$ & 6731 &  -  &   1 $\pm$ 1   & - & -  \\
\hline
\end{tabular}

\begin{tablenotes}
\item $^a$ Acording to z = 4.6891 \citep{2013A&A...559A..29C}.\\
\end{tablenotes}  
\label{tab:SMG2}
\end{table}

